Dissecting the Crab Nebula with JWST: Pulsar wind, dusty filaments, and Ni/Fe abundance constraints on the explosion mechanism

We present JWST observations of the Crab Nebula, the iconic remnant of the historical SN 1054. The observations include NIRCam and MIRI imaging mosaics, plus MIRI/MRS IFU spectra that probe two select locations within the ejecta filaments. We derive a high-resolution map of dust emission and show that the grains are concentrated in the innermost, high-density filaments. These dense filaments coincide with multiple synchrotron bays around the periphery of the Crab's pulsar wind nebula (PWN). We measure synchrotron spectral index changes in small-scale features within the PWN's torus region, including the well-known knot and wisp structures. The index variations are consistent with Doppler boosting of emission from particles with a broken power-law distribution, providing the first direct evidence that the curvature in the particle injection spectrum is tied to the acceleration mechanism at the termination shock. We detect multiple nickel and iron lines in the ejecta filaments and use photoionization models to derive nickel-to-iron abundance ratios that are a factor of 3-8 higher than the solar ratio. We also find that the previously reported order-of-magnitude higher Ni/Fe values from optical data are consistent with the lower values from JWST when we reanalyze the optical emission using updated atomic data and account for local extinction from dust. We discuss the implications of our results for understanding the nature of the explosion that produced the Crab Nebula and conclude that the observational properties are most consistent with a low-mass iron-core-collapse supernova, even though an electron-capture explosion cannot be ruled out.

==> acknowledgements.tex <==
This work is based on observations made with the NASA/ESA/CSA James Webb Space Telescope. The data were obtained from the Mikulski Archive for Space Telescopes at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5-03127 for JWST. These observations are associated with program \#1714. The support for the program was provided by the NASA grant JWST-GO-01714.

T.T. acknowledges support from the NASA grant JWST-GO-01714.001, NSF grant AST-2205314, and the NASA ADAP award 80NSSC23K1130. PJK acknowledges support from the Science Foundation Ireland/Irish Research Council Pathway program under Grant Number 21/PATH-S/9360.
D.M. acknowledges NSF support from grants PHY-2209451 and AST-2206532. 
J.M.L. acknowledges support from the NASA grant JWST-GO-01714.011 and from basic research funds of the Office of Naval Research.
M.M. acknowledges support in part from ADAP program grant No. 80NSSC22K0486, from the NSF grant AST-2206657 and from the HST GO program HST-GO-16656. We also thank Adam Burrows and Tianshu Wang for the productive discussion about their 3D explosions and nucleosynthesis models.
I.D.L. acknowledges funding from the Belgian Science Policy Office (BELSPO) through the PRODEX project “JWST/MIRI Science exploitation” (C4000142239) and from the European Research Council (ERC) under the European Union’s Horizon 2020 research and innovation programme DustOrigin (ERC-2019-StG-851622).
